Transfer learning for Remaining Useful Life Prediction Based on Consensus Self-Organizing Models

The traditional paradigm for developing machine prognostics usually relies on generalization from data acquired in experiments under controlled conditions prior to deployment of the equipment. Detecting or predicting failures and estimating machine health in this way assumes that future field data will have a very similar distribution to the experiment data. However, many complex machines operate under dynamic environmental conditions and are used in many different ways. This makes collecting comprehensive data very challenging, and the assumption that pre-deployment data and post-deployment data follow very similar distributions is unlikely to hold. Transfer Learning (TL) refers to methods for transferring knowledge learned in one setting (the source domain) to another setting (the target domain). In this work, we present a TL method for predicting Remaining Useful Life (RUL) of equipment, under the assumption that labels are available only for the source domain and not the target domain. This setting corresponds to generalizing from a limited number of run-to-failure experiments performed prior to deployment into making prognostics with data coming from deployed equipment that is being used under multiple new operating conditions and experiencing previously unseen faults. We employ a deviation detection method, Consensus Self-Organizing Models (COSMO), to create transferable features for building the RUL regression model. These features capture how different target equipment is in comparison to its peers. The efficiency of the proposed TL method is demonstrated using the NASA Turbofan Engine Degradation Simulation Data Set. Models using the COSMO transferable features show better performance than other methods on predicting RUL when the target domain is more complex than the source domain.

==> figure/cosmo_feature.tex <==

\newcommand{\tableSubplotSizeA}{0.25}
\begin{table*}
\begin{center}
\begin{tabular}{l*{3}{c}}
\toprule
& Sensor Data $x$ & COSMO Knn $\theta(ST, ST)$ & COSMO Knn $\theta(S, T)$ \\
%\hline%
\midrule
\shortstack[l]{$x_{49} \in X_S$} &
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_00.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_01.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_02.pdf}
    \end{minipage}&
\shortstack[l]{$x_{20} \in X_S$} &
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_30.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_31.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_32.pdf}
    \end{minipage}&
\shortstack[l]{$\hat{y_{20}} \in Y_S$} &
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_40.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_41.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_44.pdf}
    \end{minipage}& \midrule
\shortstack[l]{$x_{49} \in X_T$} &
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_10.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_11.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_14.pdf}
    \end{minipage}& 
\shortstack[l]{$\hat{y_{49}} \in Y_T$} &
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_20.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_21.pdf}
    \end{minipage}& 
\begin{minipage}{\tableSubplotSizeA\textwidth}
      \includegraphics[width=\textwidth]{figure/result/cosmo_feature_and_prediction_case/_24.pdf}
    \end{minipage}& \bottomrule
\end{tabular}\caption[l]{Illustration of COSMO features}
\label{tab:Dataset}
\end{center}
\end{table*} 


